An Examination of Grouping and Spatial Organization Tasks for High-Dimensional Data Exploration

How do analysts think about grouping and spatial operations? This overarching question incorporates a number of points for investigation, including understanding how analysts begin to explore a dataset, the types of grouping/spatial structures created and the operations performed on them, the relationship between grouping and spatial structures, the decisions analysts make when exploring individual observations, and the role of external information. This work contributes the design and results of such a study, in which a group of participants are asked to organize the data contained within an unfamiliar quantitative dataset. We identify several overarching approaches taken by participants to design their organizational space, discuss the interactions performed by the participants, and propose design recommendations to improve the usability of future high-dimensional data exploration tools that make use of grouping (clustering) and spatial (dimension reduction) operations.

==> tblAnimals.tex <==
\begin{table}[!b]
  \renewcommand{\arraystretch}{1.1}
  \caption{The dataset used in this study.}
  \label{tbl:userstudyanimals}
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{ l | c | c | c | c | c }
      \textbf{Animal}  &  \textbf{Furry}  &  \textbf{Big}  &  \textbf{Swims}  &  \textbf{Fierce}  &  \textbf{Solitary}  \\
      \hline
      Bat  &  39  &  1  &  0  &  33  &  20 \\
      Blue Whale  &  0  &  87  &  72  &  8  &  26 \\
      Bobcat  &  65  &  20  &  0  &  72  &  59 \\
      Cow  &  32  &  68  &  0  &  3  &  5 \\
      Deer  &  52  &  40  &  0  &  0  &  7 \\
      Giraffe  &  17  &  78  &  0  &  1  &  10 \\
      Grizzly Bear  &  82  &  87  &  3  &  62  &  59 \\
      Hippopotamus  &  0  &  79  &  40  &  19  &  25 \\
      Killer Whale  &  1  &  91  &  91  &  38  &  16 \\
      Leopard  &  43  &  55  &  5  &  70  &  34 \\
      Moose  &  37  &  88  &  3  &  9  &  32 \\
      Otter  &  47  &  11  &  85  &  6  &  31 \\
      Polar Bear  &  82  &  85  &  39  &  70  &  49 \\
      Seal  &  20  &  31  &  82  &  14  &  6 \\
      Squirrel  &  79  &  3  &  4  &  8  &  23 \\
      Walrus  &  19  &  76  &  77  &  20  &  11 \\
      Wolf  &  67  &  40  &  0  &  76  &  41 \\
    \end{tabular}
  }
\end{table}
